Symmetries of degenerate center singularities of plane vector fields

Let $D$ be a closed unit $2$-disk on the plane centered at the origin $O$, and $F$ be a smooth vector field such that $O$ is a unique singular point of $F$ and all other orbits of $F$ are simple closed curves wrapping once around $O$. Thus topologically $O$ is a "center" singularity. Let also $\mathrm{Diff}(F)$ be the group of all diffeomorphisms of $D$ which preserve orientation and orbits of $F$. In arXiv:0907.0359 the author described the homotopy type of $\mathrm{Diff}(F)$ under assumption that the $1$-jet of $F$ at $O$ is non-degenerate. In this paper degenerate case is considered. Under additional "non-degeneracy assumptions" on $F$ the path components of $\mathrm{Diff}(F)$ with respect to distinct weak topologies are described.

==> macro.tex <==
% -------- begin myemph --------------------
\makeatletter
\newcommand\testshape{family=\f@family; series=\f@series; shape=\f@shape.}
\def\myemphInternal#1{\if n\f@shape%
\begingroup\itshape #1\endgroup\/%
\else\begingroup\bfseries #1\endgroup%
\fi}
\def\myemph{\futurelet\testchar\MaybeOptArgmyemph}
\def\MaybeOptArgmyemph{\ifx[\testchar \let\next\OptArgmyemph
                 \else \let\next\NoOptArgmyemph \fi \next}
\def\OptArgmyemph[#1]#2{\index{#1}\myemphInternal{#2}}
\def\NoOptArgmyemph#1{\myemphInternal{#1}}
\makeatother
% -------- end myemph --------------------

%\swapnumbers
\theoremstyle{plain}
\newtheorem{theorem}[subsection]{Theorem}
\newtheorem{lemma}[subsection]{Lemma}
\newtheorem{proposition}[subsection]{Proposition}
\newtheorem{corollary}[subsection]{Corollary}
\newtheorem{claim}[subsection]{Claim}

%\theoremstyle{remark}
\newtheorem{remark}[subsection]{Remark}
\newtheorem{example}[subsection]{Example}

\theoremstyle{definition}
\newtheorem{definition}[subsection]{Definition}



\makeatletter
%\@addtoreset{subsection}{section}
%\@addtoreset{subsubsection}{section}
\@addtoreset{equation}{section}
\@addtoreset{figure}{section}
\@addtoreset{table}{section}
\makeatother
\renewcommand\theequation{\thesection.\arabic{equation}}

\providecommand\eqref[1]{(\ref{#1})}
\newcommand\proofstyle[1]{{\it #1}} %{\AMSPROC{\sc #1}\else{\bf #1}\fi}
\providecommand\proof{\proofstyle{Proof.~}}


\newcommand\CCC{{\mathbb C}}
\newcommand\NNN{{\mathbb N}}
\newcommand\QQQ{{\mathbb Q}}
\newcommand\RRR{{\mathbb R}}
\newcommand\ZZZ{{\mathbb Z}}


\newcommand\XX{\mathcal{X}}

\newcommand\id{\mathrm{id}}
\newcommand\diam{\mathrm{diam}}
\newcommand\im{\mathrm{im}}
\newcommand\IM{\mathrm{Im}}
\newcommand\Int{\mathrm{Int}}
\newcommand\Per{\mathrm{Per}}
\newcommand\supp{\mathrm{supp\,}}
\newcommand\Fix{\mathrm{Fix\,}}
\newcommand\interior{\mathrm{Int}}

\newcommand\grad{\triangledown} %{\mathbf{grad\,}}
\newcommand\sgrad{\mathbf{sgrad\,}}

\newcommand\rank{rank} %{\mathrm{rank}}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\AFld{F}
\newcommand\AFlow{\mathbf{F}}

\newcommand\BFld{G}
\newcommand\BFlow{\mathbf{G}}


\newcommand\ShA{\varphi}
\newcommand\imShA{Sh(\AFld)}
\newcommand\ShB{\psi}
\newcommand\imShB{Sh(\BFld)}




\newcommand\EA{\mathcal{E}(\AFld)}
\newcommand\EApl{\mathcal{E}^{+}(\AFld)}
\newcommand\EAd{\mathcal{E}^{\partial}(\AFld)}

\newcommand\DA{\mathcal{D}(\AFld)}
\newcommand\DApl{\mathcal{D}^{+}(\AFld)}
\newcommand\DAd{\mathcal{D}^{\partial}(\AFld)}



\newcommand\EidA{\mathcal{E}_{\id}(\AFld)}
\newcommand\EidApl{\mathcal{E}_{\id}^{+}(\AFld)}
\newcommand\EidAd{\mathcal{E}_{\id}^{\partial}(\AFld)}

\newcommand\DidA{\mathcal{D}_{\id}(\AFld)}
\newcommand\DidApl{\mathcal{D}_{\id}^{+}(\AFld)}
\newcommand\DidAd{\mathcal{D}_{\id}^{\partial}(\AFld)}

\newcommand\GLR[1]{\mathrm{GL}(#1,\RRR)}
\newcommand\GLRpl[1]{\mathrm{GL}^{+}(#1,\RRR)}

\newcommand\jet{\mathsf{j}}%{j^1_{\orig}}
\newcommand\jetinv{\jet^{-1}}%{\mathsf{j}}%{j^1_{\orig}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\Cinf{C^{\infty}}
\newcommand\Ci[2]{\Cinf(#1,#2)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\afunc{\alpha}
\newcommand\bfunc{\beta}
\newcommand\eps{\varepsilon}


\newcommand\func{f}
\newcommand\canon[1]{\mathsf{c}_{#1}}
\newcommand\cls[1]{[#1]}

\newcommand\dif{h}
\newcommand\gdif{g}

\newcommand\orig{O}
\newcommand\disk{D^2}
\newcommand\disko{\disk\setminus\orig}


\newcommand\Mman{M}
\newcommand\Uman{U}
\newcommand\Vman{V}


\newcommand\EAr[1]{\EA^{#1}}
\newcommand\EAplr[1]{\EApl^{#1}}
\newcommand\EAdr[1]{\EAd^{#1}}
\newcommand\DAr[1]{\DA^{#1}}
\newcommand\DAplr[1]{\DApl^{#1}}
\newcommand\DAdr[1]{\DAd^{#1}}

\newcommand\EidAr[1]{\EidA^{#1}}
\newcommand\EidAplr[1]{\EidApl^{#1}}
\newcommand\EidAdr[1]{\EidAd^{#1}}
\newcommand\DidAr[1]{\DidA^{#1}}
\newcommand\DidAplr[1]{\DidApl^{#1}}
\newcommand\DidAdr[1]{\DidAd^{#1}}


\newcommand\EB{\mathcal{E}(\BFld)}
\newcommand\EBr[1]{\EB^{#1}}
\newcommand\EidBr[1]{\mathcal{E}_{\id}(\BFld)^{#1}}


\newcommand\NFZ{{\rm(1)}}
\newcommand\NFS{{\rm(2)}}
\newcommand\NFN{{\rm(3)}}


\newcommand\Ksp{\mathbf{K}} % space K
\newcommand\Ldf{\mathbf{L}} % subset mapped to diffeomorphisms DA
\newcommand\Kpc{\mathbf{P}} % path connected subset mapped to EApl
\newcommand\Zsp{\mathbf{Z}} % path connected subset mapped to EApl


